Graph-Guided Textual Explanation Generation Framework

Natural language explanations (NLEs) are commonly used to provide plausible free-text explanations of a model's reasoning about its predictions. However, recent work has questioned their faithfulness, as they may not accurately reflect the model's internal reasoning process regarding its predicted answer. In contrast, highlight explanations--input fragments critical for the model's predicted answers--exhibit measurable faithfulness. Building on this foundation, we propose G-Tex, a Graph-Guided Textual Explanation Generation framework designed to enhance the faithfulness of NLEs. Specifically, highlight explanations are first extracted as faithful cues reflecting the model's reasoning logic toward answer prediction. They are subsequently encoded through a graph neural network layer to guide the NLE generation, which aligns the generated explanations with the model's underlying reasoning toward the predicted answer. Experiments on T5 and BART using three reasoning datasets show that G-Tex improves NLE faithfulness by up to 12.18% compared to baseline methods. Additionally, G-Tex generates NLEs with greater semantic and lexical similarity to human-written ones. Human evaluations show that G-Tex can decrease redundant content and enhance the overall quality of NLEs. Our work presents a novel method for explicitly guiding NLE generation to enhance faithfulness, serving as a foundation for addressing broader criteria in NLE and generated text.

==> eval_table.tex <==
\begin{table*}[!htbp]
    \centering
    %\fontsize{7pt}{7pt}\selectfont
\resizebox{\textwidth}{!}{
\begin{tabular}{llll}
\toprule
         \textbf{Aspects} & \textbf{Source} & \textbf{Detail}  \\
        \midrule
         Lexical overlap & ROUGE-variant  \cite{lin-2004-rouge}  & \textit{ROUGE-1} matching the texts through computing the unigram overlap; \textit{ROUGE-L} leveraging the longest common subsequence \\
     \multirow{2}{*}{Semantic overlap} & BERTScore \cite{bert-score} & measuring semantic overlap through calculating the token similarity \\
         & MoverScore \cite{zhao-etal-2019-moverscore} & measuring semantic overlap utilizing Word Mover’s distance \\
         Generation-based & BARTScore \cite{NEURIPS2021_e4d2b6e6} &  metric based on text generation using BART\\
         NLI-based  & MENLI \cite{chen2022menli} & metric based on natural language inference\\
         Discourse-based & DiscoScore \cite{zhao-etal-2023-discoscore} &  metric using BERT to model discourse coherence\\
    \bottomrule
    \end{tabular}
    }
    \caption{Details of the evaluation strategies.}
    \label{tab:eval}
\end{table*}

==> old_tables.tex <==
\begin{table*}[ht]
\centering
\small
\normalsize
\scalebox{0.71}{
\begin{tabular}{cc|ccc|cc|cccc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{Evaluation Metrics}}                                                                      & \multicolumn{3}{c|}{Faithfulness(\% $\downarrow$)}                                                                                                                      & \multicolumn{2}{c|}{Automatic Evaluation($\uparrow$)}                                                                                        & \multicolumn{4}{c}{Human Evaluation(1-7 $\uparrow$)}                                                                                                                                               \\ \cline{3-11} 
\multicolumn{2}{c|}{}                                                                                                         & \multicolumn{1}{c|}{Counter} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} & \multicolumn{1}{c|}{Coverage} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Non\\ Redund.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Non\\ Contrad.\end{tabular}} & Overall \\ \hline
\multicolumn{2}{c|}{Fine-tuning}                                                                                              & \multicolumn{1}{c|}{35.87}   & \multicolumn{1}{c|}{47.08}                                                     & 16.89                                                   & \multicolumn{1}{c|}{15.430}                                                      & 0.894                                                     & \multicolumn{1}{c|}{6.72}     & \multicolumn{1}{c|}{5.86}                                                  & \multicolumn{1}{c|}{6.67}                                                   & 6.28    \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Highlight Token \\ Explanation\end{tabular}}}    & Prompt      & \multicolumn{1}{c|}{33.57}        & \multicolumn{1}{c|}{42.04}                                                          &             14.11                                            & \multicolumn{1}{c|}{}                                                            &                                                           & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}                                                      & \multicolumn{1}{c|}{}                                                       &         \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                           & GAT (Ours)  & \multicolumn{1}{c|}{31.40}   & \multicolumn{1}{c|}{35.92}                                                     & 11.28                                                   & \multicolumn{1}{c|}{16.387}                                                      & 0.907                                                     & \multicolumn{1}{c|}{6.74}     & \multicolumn{1}{c|}{5.80}                                                  & \multicolumn{1}{c|}{6.67}                                                   & 6.06    \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                           & GCN (Ours)  & \multicolumn{1}{c|}{30.67}   & \multicolumn{1}{c|}{35.47}                                                     & 10.88                                                   & \multicolumn{1}{c|}{16.409}                                                      & 0.908                                                     & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}                                                      & \multicolumn{1}{c|}{}                                                       &         \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                           & SAGE (Ours) & \multicolumn{1}{c|}{31.29}   & \multicolumn{1}{c|}{33.45}                                                     & 10.47                                                   & \multicolumn{1}{c|}{16.426}                                                      & 0.908                                                     & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}                                                      & \multicolumn{1}{c|}{}                                                       &         \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Token Interactive\\   Explanation\end{tabular}}} & Prompt      & \multicolumn{1}{c|}{37.25}        & \multicolumn{1}{c|}{51.56}                                                          &            19.20                                             & \multicolumn{1}{c|}{}                                                            &                                                           & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}                                                      & \multicolumn{1}{c|}{}                                                       &         \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                           & GAT (Ours)  & \multicolumn{1}{c|}{31.14}   & \multicolumn{1}{c|}{34.28}                                                     & 10.67                                                   & \multicolumn{1}{c|}{16.387}                                                      & 0.907                                                     & \multicolumn{1}{c|}{6.75}     & \multicolumn{1}{c|}{5.95}                                                  & \multicolumn{1}{c|}{6.64}                                                   & 6.37    \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                           & GCN (Ours)  & \multicolumn{1}{c|}{30.77}   & \multicolumn{1}{c|}{32.59}                                                     & 10.03                                                   & \multicolumn{1}{c|}{16.422}                                                      & 0.907                                                     & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}                                                      & \multicolumn{1}{c|}{}                                                       &         \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                           & SAGE (Ours) & \multicolumn{1}{c|}{30.87}   & \multicolumn{1}{c|}{33.68}                                                     & 10.40                                                   & \multicolumn{1}{c|}{16.443}                                                      & 0.908                                                     & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}                                                      & \multicolumn{1}{c|}{}                                                       &         \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Span Interactive\\  Explanation\end{tabular}}}   & Prompt      & \multicolumn{1}{c|}{32.14}        & \multicolumn{1}{c|}{42.47}                                                          &          13.65                                               & \multicolumn{1}{c|}{}                                                            &                                                           & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}                                                      & \multicolumn{1}{c|}{}                                                       &         \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                           & GAT (Ours)  & \multicolumn{1}{c|}{31.68}   & \multicolumn{1}{c|}{38.05}                                                     & 12.05                                                   & \multicolumn{1}{c|}{16.400}                                                      & 0.907                                                     & \multicolumn{1}{c|}{6.67}     & \multicolumn{1}{c|}{5.92}                                                  & \multicolumn{1}{c|}{6.72}                                                   & 6.26    \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                           & GCN (Ours)  & \multicolumn{1}{c|}{31.54}   & \multicolumn{1}{c|}{34.31}                                                     & 10.82                                                   & \multicolumn{1}{c|}{16.444}                                                      & 0.907                                                     & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}                                                      & \multicolumn{1}{c|}{}                                                       &         \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                           & SAGE (Ours) & \multicolumn{1}{c|}{31.24}   & \multicolumn{1}{c|}{32.07}                                                     & 10.02                                                   & \multicolumn{1}{c|}{16.277}                                                      & 0.907                                                     & \multicolumn{1}{c|}{}         & \multicolumn{1}{c|}{}                                                      & \multicolumn{1}{c|}{}                                                       &         \\ \hline
\end{tabular}
}
\caption{Overall Evaluation Results on e-SNLI of T5-based \method. The best performance of each evaluation metric across all NLE generation models is in bold.}
\label{tab:all_results_esnli_t5}
\end{table*}


\begin{table*}[ht]
\centering
\small
\normalsize
\scalebox{0.71}{
\begin{tabular}{cc|ccc|cc|cccc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{Evaluation Metrics}}                                                                    & \multicolumn{3}{c|}{Faithfulness(\% $\downarrow$)}                                                                                                                             & \multicolumn{2}{c|}{Automatic Evaluation($\uparrow$)}                                                                                        & \multicolumn{4}{c}{Human Evaluation(1-7 $\uparrow$)}                                                                                                                                                                 \\ \cline{3-11} 
\multicolumn{2}{c|}{}                                                                                                       & \multicolumn{1}{c|}{Counter}        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (1-100)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} & \multicolumn{1}{c|}{Coverage}      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Non\\ Redund.\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Non\\ Contrad.\end{tabular}} & Overall              \\ \hline
\multicolumn{2}{c|}{Fine-tuning}                                                                                            & \multicolumn{1}{c|}{50.25}          & \multicolumn{1}{c|}{49.34}                                                     & 24.80                                                   & \multicolumn{1}{c|}{15.755}                                                      & \textbf{0.892}                                            & \multicolumn{1}{c|}{\textbf{5.66}} & \multicolumn{1}{c|}{4.41}                                                  & \multicolumn{1}{c|}{4.91}                                                   & 5.53                 \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Highlight Token \\ Explanation\end{tabular}}}  & Prompt      & \multicolumn{1}{c|}{54.27}               & \multicolumn{1}{c|}{46.56}                                                          & \multicolumn{1}{c|}{25.27}                                   & \multicolumn{1}{l|}{}                                                            & \multicolumn{1}{l|}{}                                     & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}                                                      & \multicolumn{1}{l|}{}                                                       & \multicolumn{1}{l}{} \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                         & GAT (Ours)  & \multicolumn{1}{c|}{49.12}          & \multicolumn{1}{c|}{44.76}                                                     & 21.99                                                   & \multicolumn{1}{c|}{15.724}                                                      & \textbf{0.892}                                            & \multicolumn{1}{c|}{5.08}          & \multicolumn{1}{c|}{4.27}                                                  & \multicolumn{1}{c|}{4.51}                                                   & 5.20                 \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                         & GCN (Ours)  & \multicolumn{1}{c|}{50.82}          & \multicolumn{1}{c|}{49.61}                                                     & 25.21                                                   & \multicolumn{1}{c|}{15.583}                                                      & 0.891                                                     & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{-}                                                     & \multicolumn{1}{c|}{-}                                                      & -                    \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                         & SAGE (Ours) & \multicolumn{1}{c|}{49.41}          & \multicolumn{1}{c|}{45.42}                                                     & 22.44                                                   & \multicolumn{1}{c|}{15.649}                                                      & 0.891                                                     & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{-}                                                     & \multicolumn{1}{c|}{-}                                                      & -                    \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Token Interactive\\ Explanation\end{tabular}}} & Prompt      & \multicolumn{1}{c|}{64.92}               & \multicolumn{1}{c|}{51.29}                                                          & \multicolumn{1}{c|}{33.30}                                   & \multicolumn{1}{l|}{}                                                            & \multicolumn{1}{l|}{}                                     & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}                                                      & \multicolumn{1}{l|}{}                                                       & \multicolumn{1}{l}{} \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                         & GAT (Ours)  & \multicolumn{1}{c|}{49.29}          & \multicolumn{1}{c|}{43.49}                                                     & 21.44                                                   & \multicolumn{1}{c|}{15.665}                                                      & 0.891                                                     & \multicolumn{1}{c|}{5.60}          & \multicolumn{1}{c|}{\textbf{4.81}}                                         & \multicolumn{1}{c|}{\textbf{5.08}}                                          & 5.61                 \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                         & GCN (Ours)  & \multicolumn{1}{c|}{48.78}          & \multicolumn{1}{c|}{\textbf{43.42}}                                            & \textbf{21.18}                                          & \multicolumn{1}{c|}{15.792}                                                      & \textbf{0.892}                                            & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{-}                                                     & \multicolumn{1}{c|}{-}                                                      & -                    \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                         & SAGE (Ours) & \multicolumn{1}{c|}{49.19}          & \multicolumn{1}{c|}{44.20}                                                     & 21.74                                                   & \multicolumn{1}{c|}{15.712}                                                      & 0.891                                                     & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{-}                                                     & \multicolumn{1}{c|}{-}                                                      & -                    \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Span Interactive\\ Explanation\end{tabular}}}  & Prompt      & \multicolumn{1}{c|}{56.21}               & \multicolumn{1}{c|}{50.20}                                                          & \multicolumn{1}{c|}{28.22}                                   & \multicolumn{1}{l|}{}                                                            & \multicolumn{1}{l|}{}                                     & \multicolumn{1}{l|}{}              & \multicolumn{1}{l|}{}                                                      & \multicolumn{1}{l|}{}                                                       & \multicolumn{1}{l}{} \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                         & GAT (Ours)  & \multicolumn{1}{c|}{48.46}          & \multicolumn{1}{c|}{49.22}                                                     & 23.85                                                   & \multicolumn{1}{c|}{16.118}                                                      & \textbf{0.892}                                            & \multicolumn{1}{c|}{5.65}          & \multicolumn{1}{c|}{4.67}                                                  & \multicolumn{1}{c|}{4.90}                                                   & \textbf{5.63}        \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                         & GCN (Ours)  & \multicolumn{1}{c|}{49.36}          & \multicolumn{1}{c|}{50.46}                                                     & 24.91                                                   & \multicolumn{1}{c|}{16.180}                                                      & \textbf{0.892}                                            & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{-}                                                     & \multicolumn{1}{c|}{-}                                                      & -                    \\ \cline{2-11} 
\multicolumn{1}{c|}{}                                                                                         & SAGE (Ours) & \multicolumn{1}{c|}{\textbf{48.01}} & \multicolumn{1}{c|}{46.87}                                                     & 22.50                                                   & \multicolumn{1}{c|}{\textbf{16.191}}                                             & \textbf{0.892}                                            & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{-}                                                     & \multicolumn{1}{c|}{-}                                                      & -                    \\ \hline
\end{tabular}
}
\caption{Overall Evaluation Results on ECQA of T5-based \method . The best performance of each evaluation metric across all NLE generation models is in bold.}
\label{tab:all_results_ecqa_t5}
\end{table*}



\begin{table*}[ht]
\centering
\small
\normalsize
\scalebox{0.72}{
\begin{tabular}{cc|cccc|cccc}
\hline
\multicolumn{2}{c|}{Datasets} &
  \multicolumn{4}{c|}{e-SNLI} &
  \multicolumn{4}{c}{ComVE} \\ \hline
\multicolumn{2}{c|}{\multirow{2}{*}{Evaluation Metrics}} &
  \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
  \multicolumn{2}{c|}{Automatic Evaluation($\uparrow$)} &
  \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
  \multicolumn{2}{c}{Automatic Evaluation($\uparrow$)} \\ \cline{3-10} 
\multicolumn{2}{c|}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} \\ \hline
\multicolumn{2}{c|}{Fine-tuning} &
  \multicolumn{1}{c|}{47.08} &
  \multicolumn{1}{c|}{16.89} &
  \multicolumn{1}{c|}{15.430} &
  0.894 &
  \multicolumn{1}{c|}{\textbf{87.17}} &
  \multicolumn{1}{c|}{73.73} &
  \multicolumn{1}{c|}{-} &
  - \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Highlight Token \\ Explanation\end{tabular}}} &
  Prompt &
  \multicolumn{1}{c|}{42.04} &
  \multicolumn{1}{c|}{14.11} &
  \multicolumn{1}{c|}{15.686} &
  0.898 &
  \multicolumn{1}{c|}{87.04} &
  \multicolumn{1}{c|}{74.18} &
  \multicolumn{1}{c|}{-} &
  - \\ \cline{2-10} 
\multicolumn{1}{c|}{} &
  \sage (Ours) &
  \multicolumn{1}{c|}{33.45} &
  \multicolumn{1}{c|}{10.47} &
  \multicolumn{1}{c|}{16.426} &
  \textbf{0.908} &
  \multicolumn{1}{c|}{90.44} &
  \multicolumn{1}{c|}{\textbf{56.59}} &
  \multicolumn{1}{c|}{-} &
  - \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Token Interactive\\ Explanation\end{tabular}}} &
  Prompt &
  \multicolumn{1}{c|}{51.56} &
  \multicolumn{1}{c|}{19.20} &
  \multicolumn{1}{c|}{15.478} &
  0.898 &
  \multicolumn{1}{c|}{87.36} &
  \multicolumn{1}{c|}{76.43} &
  \multicolumn{1}{c|}{-} &
  - \\ \cline{2-10} 
\multicolumn{1}{c|}{} &
  \sage (Ours) &
  \multicolumn{1}{c|}{33.68} &
  \multicolumn{1}{c|}{10.40} &
  \multicolumn{1}{c|}{\textbf{16.443}} &
  \textbf{0.908} &
  \multicolumn{1}{c|}{91.11} &
  \multicolumn{1}{c|}{76.41} &
  \multicolumn{1}{c|}{-} &
  - \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Span Interactive\\ Explanation\end{tabular}}} &
  Prompt &
  \multicolumn{1}{c|}{42.47} &
  \multicolumn{1}{c|}{13.65} &
  \multicolumn{1}{c|}{16.031} &
  0.899 &
  \multicolumn{1}{c|}{89.34} &
  \multicolumn{1}{c|}{79.44} &
  \multicolumn{1}{c|}{-} &
  - \\ \cline{2-10} 
\multicolumn{1}{c|}{} &
  \sage (Ours) &
  \multicolumn{1}{c|}{\textbf{32.07}} &
  \multicolumn{1}{c|}{\textbf{10.02}} &
  \multicolumn{1}{c|}{16.277} &
  0.907 &
  \multicolumn{1}{c|}{92.15} &
  \multicolumn{1}{c|}{70.97} &
  \multicolumn{1}{c|}{-} &
  - \\ \hline
\end{tabular}
}
\caption{Overall Evaluation Results on e-SNLI and ComVE datasets of T5-based \sage (Our \method model with \sage as the graph layer). The best performance of each evaluation metric across all NLE generation models is in bold. \textcolor{red}{See Appendix X for results on ECQA dataset}.}
\label{tab:all_results_esnli_and_ComVE_t5}
\end{table*}


\begin{table*}[ht]
\centering
\small
\normalsize
\scalebox{0.72}{
\begin{tabular}{cc|cccc|cccc}
\hline
\multicolumn{2}{c|}{Datasets} &
  \multicolumn{4}{c|}{e-SNLI} &
  \multicolumn{4}{c}{ComVE} \\ \hline
\multicolumn{2}{c|}{\multirow{2}{*}{Evaluation Metrics}} &
  \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
  \multicolumn{2}{c|}{Automatic Evaluation($\uparrow$)} &
  \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
  \multicolumn{2}{c}{Automatic Evaluation($\uparrow$)} \\ \cline{3-10} 
\multicolumn{2}{c|}{} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} \\ \hline
\multicolumn{2}{c|}{Fine-tuning} &
  \multicolumn{1}{c|}{57.98} &
  \multicolumn{1}{c|}{19.64} &
  \multicolumn{1}{c|}{15.732} &
  0.906 &
  \multicolumn{1}{c|}{\textbf{82.72}} &
  \multicolumn{1}{c|}{72.82} &
  \multicolumn{1}{c|}{-} &
  - \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Highlight Token \\ Explanation\end{tabular}}} &
  Prompt &
  \multicolumn{1}{c|}{56.65} &
  \multicolumn{1}{c|}{24.20} &
  \multicolumn{1}{c|}{15.678} &
  0.898 &
  \multicolumn{1}{c|}{84.74} &
  \multicolumn{1}{c|}{61.97} &
  \multicolumn{1}{c|}{-} &
  - \\ \cline{2-10} 
\multicolumn{1}{c|}{} &
  \sage (Ours) &
  \multicolumn{1}{c|}{46.36} &
  \multicolumn{1}{c|}{\textbf{14.37}} &
  \multicolumn{1}{c|}{16.318} &
  \textbf{0.909} &
  \multicolumn{1}{c|}{92.99} &
  \multicolumn{1}{c|}{\textbf{57.81}} &
  \multicolumn{1}{c|}{-} &
  - \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Token Interactive\\ Explanation\end{tabular}}} &
  Prompt &
  \multicolumn{1}{c|}{51.56} &
  \multicolumn{1}{c|}{19.20} &
  \multicolumn{1}{c|}{15.478} &
  0.898 &
  \multicolumn{1}{c|}{95.85} &
  \multicolumn{1}{c|}{69.86} &
  \multicolumn{1}{c|}{-} &
  - \\ \cline{2-10} 
\multicolumn{1}{c|}{} &
  \sage (Ours) &
  \multicolumn{1}{c|}{47.55} &
  \multicolumn{1}{c|}{15.55} &
  \multicolumn{1}{c|}{\textbf{16.427}} &
  \textbf{0.909} &
  \multicolumn{1}{c|}{97.18} &
  \multicolumn{1}{c|}{72.52} &
  \multicolumn{1}{c|}{-} &
  - \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Span Interactive\\ Explanation\end{tabular}}} &
  Prompt &
  \multicolumn{1}{c|}{51.10} &
  \multicolumn{1}{c|}{17.41} &
  \multicolumn{1}{c|}{16.027} &
  \textbf{0.909} &
  \multicolumn{1}{c|}{94.89} &
  \multicolumn{1}{c|}{65.52} &
  \multicolumn{1}{c|}{-} &
  - \\ \cline{2-10} 
\multicolumn{1}{c|}{} &
  \sage (Ours) &
  \multicolumn{1}{c|}{\textbf{44.42}} &
  \multicolumn{1}{c|}{14.56} &
  \multicolumn{1}{c|}{16.517} &
  \textbf{0.909} &
  \multicolumn{1}{c|}{85.50} &
  \multicolumn{1}{c|}{64.21} &
  \multicolumn{1}{c|}{-} &
  - \\ \hline
\end{tabular}
}
\caption{Overall Evaluation Results on e-SNLI and ComVE datasets of BART-based \sage (Our \method model with \sage as the graph layer). The best performance of each evaluation metric across all NLE generation models is in bold. \textcolor{red}{See Appendix X for results on ECQA dataset}.}
\label{tab:all_results_esnli_and_ComVE_bart}
\end{table*}





% \begin{table*}[ht]
% \centering
% \scalebox{0.40}{
% \begin{tabular}{@{}c c|cccc|cccc|cccc|cccc@{}}
% \toprule
% \multirow{3}{*}{\textbf{Explanation Type}} & \multirow{3}{*}{\textbf{Model}} 
% & \multicolumn{8}{c|}{\textbf{T5-based}} 
% & \multicolumn{8}{c}{\textbf{BART-based}} \\ 
% \cmidrule(lr){3-10}\cmidrule(lr){11-18}
% & & \multicolumn{4}{c|}{e-SNLI} & \multicolumn{4}{c|}{ComVE}
% & \multicolumn{4}{c|}{e-SNLI} & \multicolumn{4}{c}{ComVE} \\
% \cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}\cmidrule(lr){15-18}
% & & \multicolumn{2}{c}{Unfaithfulness(\%$\downarrow$)} & \multicolumn{2}{c|}{Automatic($\uparrow$)}
% & \multicolumn{2}{c}{Unfaithfulness(\%$\downarrow$)} & \multicolumn{2}{c|}{Automatic($\uparrow$)}
% & \multicolumn{2}{c}{Unfaithfulness(\%$\downarrow$)} & \multicolumn{2}{c|}{Automatic($\uparrow$)}
% & \multicolumn{2}{c}{Unfaithfulness(\%$\downarrow$)} & \multicolumn{2}{c}{Automatic($\uparrow$)} \\
% & & Counter & Total & SacreBLEU & BERTScore & Counter & Total & SacreBLEU & BERTScore 
% & Counter & Total & SacreBLEU & BERTScore & Counter & Total & SacreBLEU & BERTScore \\
% \midrule
% % None - Fine-tuning
% None & Fine-tuning &
% 47.08 & 16.89 & 15.430 & 0.894 & 87.17 & 73.73 & - & - &
% 57.98 & 19.64 & 15.732 & 0.906 & \textbf{82.72} & 72.82 & - & - \\
% \midrule
% % Highlight Token: Prompt
% \multirow{2}{*}{Highlight Token} & Prompt &
% 42.04 & 14.11 & 15.686 & 0.898 & 87.04 & 74.18 & - & - &
% 56.65 & 24.20 & 15.678 & 0.898 & 84.74 & 61.97 & - & - \\
% % Highlight Token: SAGE Ours
% & \sage (Ours) &
% 33.45 & 10.47 & 16.426 & \textbf{0.908} & 90.44 & \textbf{56.59} & - & - &
% 46.36 & \textbf{14.37} & 16.318 & \textbf{0.909} & 92.99 & \textbf{57.81} & - & - \\
% \midrule
% % Token Interactions: Prompt
% \multirow{2}{*}{Token Interactions} & Prompt &
% 51.56 & 19.20 & 15.478 & 0.898 & 87.36 & 76.43 & - & - &
% 51.56 & 19.20 & 15.478 & 0.898 & 95.85 & 69.86 & - & - \\
% % Token Interactions: SAGE Ours
% & \sage (Ours) &
% 33.68 & 10.40 & \textbf{16.443} & \textbf{0.908} & 91.11 & 76.41 & - & - &
% 47.55 & 15.55 & \textbf{16.427} & \textbf{0.909} & 97.18 & 72.52 & - & - \\
% \midrule
% % Span Interactions: Prompt
% \multirow{2}{*}{Span Interactions} & Prompt &
% 42.47 & 13.65 & 16.031 & 0.899 & 89.34 & 79.44 & - & - &
% 51.10 & 17.41 & 16.027 & \textbf{0.909} & 94.89 & 65.52 & - & - \\
% % Span Interactions: SAGE Ours
% & \sage (Ours) &
% \textbf{32.07} & \textbf{10.02} & 16.277 & 0.907 & 92.15 & 70.97 & - & - &
% \textbf{44.42} & 14.56 & 16.517 & \textbf{0.909} & 85.50 & 64.21 & - & - \\
% \bottomrule
% \end{tabular}
% }
% \caption{Overall evaluation results on e-SNLI and ComVE datasets for T5-based and BART-based models using \sage (our \method model with \sage as the graph layer). The best performance of each evaluation metric across all NLE generation models of the same base architecture is in bold. \textcolor{red}{See Appendix X for results on ECQA dataset}.}
% \label{tab:all_results_combined}
% \end{table*}



% \begin{table*}[ht]
% \centering
% \small
% \normalsize
% \scalebox{0.55}{
% \begin{tabular}{cc|cccc|cccc|cccc}
% \hline
% \multicolumn{2}{c|}{Datasets} &
%   \multicolumn{4}{c|}{e-SNLI} &
%   \multicolumn{4}{c|}{ECQA} &
%   \multicolumn{4}{c}{ComVE} \\ \hline
% \multicolumn{2}{c|}{\multirow{2}{*}{Evaluation Metrics}} &
%   \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
%   \multicolumn{2}{c|}{Automatic Evaluation($\uparrow$)} &
%   \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
%   \multicolumn{2}{c|}{Automatic Evaluation($\uparrow$)} &
%   \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
%   \multicolumn{2}{c}{Automatic Evaluation($\uparrow$)} \\ \cline{3-14} 
% \multicolumn{2}{c|}{} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
%   \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
%   \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
%   \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} \\ \hline
% \multicolumn{2}{c|}{Fine-tuning} &
%   \multicolumn{1}{c|}{47.08} &
%   \multicolumn{1}{c|}{16.89} &
%   \multicolumn{1}{c|}{15.430} &
%   0.894 &
%   \multicolumn{1}{c|}{49.34} &
%   \multicolumn{1}{c|}{24.80} &
%   \multicolumn{1}{c|}{14.057} &
%   0.883 &
%   \multicolumn{1}{c|}{\textbf{87.17}} &
%   \multicolumn{1}{c|}{73.73} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Highlight Token \\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{42.04} &
%   \multicolumn{1}{c|}{14.11} &
%   \multicolumn{1}{c|}{15.686} &
%   0.898 &
%   \multicolumn{1}{c|}{46.56} &
%   \multicolumn{1}{c|}{25.27} &
%   \multicolumn{1}{c|}{15.303} &
%   0.887 &
%   \multicolumn{1}{c|}{87.04} &
%   \multicolumn{1}{c|}{74.18} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{2-14} 
% \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{33.45} &
%   \multicolumn{1}{c|}{10.47} &
%   \multicolumn{1}{c|}{16.426} &
%   \textbf{0.908} &
%   \multicolumn{1}{c|}{45.42} &
%   \multicolumn{1}{c|}{22.44} &
%   \multicolumn{1}{c|}{13.968} &
%   0.882 &
%   \multicolumn{1}{c|}{90.44} &
%   \multicolumn{1}{c|}{\textbf{56.59}} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Token Interactive\\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{51.56} &
%   \multicolumn{1}{c|}{19.20} &
%   \multicolumn{1}{c|}{15.478} &
%   0.898 &
%   \multicolumn{1}{c|}{51.29} &
%   \multicolumn{1}{c|}{33.30} &
%   \multicolumn{1}{c|}{15.311} &
%   0.887 &
%   \multicolumn{1}{c|}{87.36} &
%   \multicolumn{1}{c|}{76.43} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{2-14} 
% \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{33.68} &
%   \multicolumn{1}{c|}{10.40} &
%   \multicolumn{1}{c|}{\textbf{16.443}} &
%   \textbf{0.908} &
%   \multicolumn{1}{c|}{\textbf{44.20}} &
%   \multicolumn{1}{c|}{\textbf{21.74}} &
%   \multicolumn{1}{c|}{13.978} &
%   0.882 &
%   \multicolumn{1}{c|}{91.11} &
%   \multicolumn{1}{c|}{76.41} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Span Interactive\\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{42.47} &
%   \multicolumn{1}{c|}{13.65} &
%   \multicolumn{1}{c|}{16.031} &
%   0.899 &
%   \multicolumn{1}{c|}{50.20} &
%   \multicolumn{1}{c|}{28.22} &
%   \multicolumn{1}{c|}{\textbf{16.046}} &
%   \textbf{0.888} &
%   \multicolumn{1}{c|}{89.34} &
%   \multicolumn{1}{c|}{79.44} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{2-14} 
% \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{\textbf{32.07}} &
%   \multicolumn{1}{c|}{\textbf{10.02}} &
%   \multicolumn{1}{c|}{16.277} &
%   0.907 &
%   \multicolumn{1}{c|}{46.87} &
%   \multicolumn{1}{c|}{22.50} &
%   \multicolumn{1}{c|}{14.509} &
%   0.884 &
%   \multicolumn{1}{c|}{92.15} &
%   \multicolumn{1}{c|}{70.97} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \hline
% \end{tabular}
% }
% \caption{Overall Evaluation Results on e-SNLI, ECQA and ComVE datasets of T5-based \sage (Our \method with \sage as the graph layer). The best performance of each evaluation metric across all NLE generation models is in bold.}
% \label{tab:all_results_all_datasets_t5}
% \end{table*}



% \begin{table*}[ht]
% \centering
% \small
% \normalsize
% \scalebox{0.55}{
% \begin{tabular}{cc|cccc|cccc|cccc}
% \hline
% \multicolumn{2}{c|}{Datasets} &
%   \multicolumn{4}{c|}{e-SNLI} &
%   \multicolumn{4}{c|}{ECQA} &
%   \multicolumn{4}{c}{ComVE} \\ \hline
% \multicolumn{2}{c|}{\multirow{2}{*}{Evaluation Metrics}} &
%   \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
%   \multicolumn{2}{c|}{Automatic Evaluation($\uparrow$)} &
%   \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
%   \multicolumn{2}{c|}{Automatic Evaluation($\uparrow$)} &
%   \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
%   \multicolumn{2}{c}{Automatic Evaluation($\uparrow$)} \\ \cline{3-14} 
% \multicolumn{2}{c|}{} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
%   \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
%   \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
%   \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} \\ \hline
% \multicolumn{2}{c|}{Fine-tuning} &
%   \multicolumn{1}{c|}{57.98} &
%   \multicolumn{1}{c|}{19.64} &
%   \multicolumn{1}{c|}{15.732} &
%   0.906 &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{12.484} &
%   0.836 &
%   \multicolumn{1}{c|}{\textbf{82.72}} &
%   \multicolumn{1}{c|}{72.82} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Highlight Token \\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{56.65} &
%   \multicolumn{1}{c|}{24.20} &
%   \multicolumn{1}{c|}{15.678} &
%   0.898 &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{10.733} &
%   0.754 &
%   \multicolumn{1}{c|}{84.74} &
%   \multicolumn{1}{c|}{61.97} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{2-14} 
% \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{46.36} &
%   \multicolumn{1}{c|}{\textbf{14.37}} &
%   \multicolumn{1}{c|}{16.318} &
%   \textbf{0.909} &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{12.659} &
%   0.836 &
%   \multicolumn{1}{c|}{92.99} &
%   \multicolumn{1}{c|}{\textbf{57.81}} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Token Interactive\\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{51.56} &
%   \multicolumn{1}{c|}{19.20} &
%   \multicolumn{1}{c|}{15.478} &
%   0.898 &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{12.724} &
%   0.837 &
%   \multicolumn{1}{c|}{95.85} &
%   \multicolumn{1}{c|}{69.86} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{2-14} 
% \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{47.55} &
%   \multicolumn{1}{c|}{15.55} &
%   \multicolumn{1}{c|}{\textbf{16.427}} &
%   \textbf{0.909} &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{\textbf{14.773}} &
%   \textbf{0.847} &
%   \multicolumn{1}{c|}{97.18} &
%   \multicolumn{1}{c|}{72.52} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Span Interactive\\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{51.10} &
%   \multicolumn{1}{c|}{17.41} &
%   \multicolumn{1}{c|}{16.027} &
%   \textbf{0.909} &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{12.288} &
%   0.835 &
%   \multicolumn{1}{c|}{94.89} &
%   \multicolumn{1}{c|}{65.52} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{2-14} 
% \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{\textbf{44.42}} &
%   \multicolumn{1}{c|}{14.56} &
%   \multicolumn{1}{c|}{16.517} &
%   \textbf{0.909} &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{100} &
%   \multicolumn{1}{c|}{12.802} &
%   0.837 &
%   \multicolumn{1}{c|}{85.50} &
%   \multicolumn{1}{c|}{64.21} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \hline
% \end{tabular}
% }
% \caption{Overall Evaluation Results on e-SNLI, ECQA and ComVE datasets of BART-based \sage (Our \method with \sage as the graph layer). The best performance of each evaluation metric across all NLE generation models is in bold.}
% \label{tab:all_results_all_datasets_bart}
% \end{table*}



% \begin{table*}[ht]
% \centering
% \small
% \normalsize
% \scalebox{0.71}{
% \begin{tabular}{lcc|cccc|cccc}
% \hline
% \multicolumn{1}{c}{} &
%   \multicolumn{2}{c|}{Datasets} &
%   \multicolumn{4}{c|}{e-SNLI} &
%   \multicolumn{4}{c}{ComVE} \\ \hline
%  &
%   \multicolumn{2}{c|}{\multirow{2}{*}{Evaluation Metrics}} &
%   \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
%   \multicolumn{2}{c|}{Automatic Evaluation($\uparrow$)} &
%   \multicolumn{2}{c|}{Unfaithfulness(\% $\downarrow$)} &
%   \multicolumn{2}{c}{Automatic Evaluation($\uparrow$)} \\ \cline{4-11} 
%  &
%   \multicolumn{2}{c|}{} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
%   \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Counter\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total\\ Unfaith\end{tabular}} &
%   \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SacreBLEU\\ (0-100)\end{tabular}} &
%   \begin{tabular}[c]{@{}c@{}}BERTScore\\ (0-1)\end{tabular} \\ \hline
% \multirow{7}{*}{T5} &
%   \multicolumn{2}{c|}{Fine-tuning} &
%   \multicolumn{1}{c|}{47.08} &
%   \multicolumn{1}{c|}{16.89} &
%   \multicolumn{1}{c|}{15.430} &
%   0.894 &
%   \multicolumn{1}{c|}{\textbf{87.17}} &
%   \multicolumn{1}{c|}{73.73} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{2-11} 
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Highlight Token \\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{42.04} &
%   \multicolumn{1}{c|}{14.11} &
%   \multicolumn{1}{c|}{15.686} &
%   0.898 &
%   \multicolumn{1}{c|}{87.04} &
%   \multicolumn{1}{c|}{74.18} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{3-11} 
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{33.45} &
%   \multicolumn{1}{c|}{10.47} &
%   \multicolumn{1}{c|}{16.426} &
%   \textbf{0.908} &
%   \multicolumn{1}{c|}{90.44} &
%   \multicolumn{1}{c|}{\textbf{56.59}} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{2-11} 
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Token Interactive\\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{51.56} &
%   \multicolumn{1}{c|}{19.20} &
%   \multicolumn{1}{c|}{15.478} &
%   0.898 &
%   \multicolumn{1}{c|}{87.36} &
%   \multicolumn{1}{c|}{76.43} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{3-11} 
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{33.68} &
%   \multicolumn{1}{c|}{10.40} &
%   \multicolumn{1}{c|}{\textbf{16.443}} &
%   \textbf{0.908} &
%   \multicolumn{1}{c|}{91.11} &
%   \multicolumn{1}{c|}{76.41} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{2-11} 
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Span Interactive\\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{42.47} &
%   \multicolumn{1}{c|}{13.65} &
%   \multicolumn{1}{c|}{16.031} &
%   0.899 &
%   \multicolumn{1}{c|}{89.34} &
%   \multicolumn{1}{c|}{79.44} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{3-11} 
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{\textbf{32.07}} &
%   \multicolumn{1}{c|}{\textbf{10.02}} &
%   \multicolumn{1}{c|}{16.277} &
%   0.907 &
%   \multicolumn{1}{c|}{92.15} &
%   \multicolumn{1}{c|}{70.97} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \hline
% \multirow{7}{*}{BART} &
%   \multicolumn{2}{c|}{Fine-tuning} &
%   \multicolumn{1}{c|}{57.98} &
%   \multicolumn{1}{c|}{19.64} &
%   \multicolumn{1}{c|}{15.732} &
%   0.906 &
%   \multicolumn{1}{c|}{\textbf{82.72}} &
%   \multicolumn{1}{c|}{72.82} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{2-11} 
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Highlight Token \\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{56.65} &
%   \multicolumn{1}{c|}{24.20} &
%   \multicolumn{1}{c|}{15.678} &
%   0.898 &
%   \multicolumn{1}{c|}{84.74} &
%   \multicolumn{1}{c|}{61.97} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{3-11} 
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{46.36} &
%   \multicolumn{1}{c|}{\textbf{14.37}} &
%   \multicolumn{1}{c|}{16.318} &
%   \textbf{0.909} &
%   \multicolumn{1}{c|}{92.99} &
%   \multicolumn{1}{c|}{\textbf{57.81}} &
%   \multicolumn{1}{c|}{\textbf{-}} &
%   - \\ \cline{2-11} 
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Token Interactive\\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{51.56} &
%   \multicolumn{1}{c|}{19.20} &
%   \multicolumn{1}{c|}{15.478} &
%   0.898 &
%   \multicolumn{1}{c|}{95.85} &
%   \multicolumn{1}{c|}{69.86} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{3-11} 
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{47.55} &
%   \multicolumn{1}{c|}{15.55} &
%   \multicolumn{1}{c|}{16.427} &
%   \textbf{0.909} &
%   \multicolumn{1}{c|}{97.18} &
%   \multicolumn{1}{c|}{72.52} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{2-11} 
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Span Interactive\\ Explanation\end{tabular}}} &
%   Prompt &
%   \multicolumn{1}{c|}{51.10} &
%   \multicolumn{1}{c|}{17.41} &
%   \multicolumn{1}{c|}{16.027} &
%   \textbf{0.909} &
%   \multicolumn{1}{c|}{94.89} &
%   \multicolumn{1}{c|}{65.52} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \cline{3-11} 
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \multicolumn{1}{c|}{\textbf{44.42}} &
%   \multicolumn{1}{c|}{14.56} &
%   \multicolumn{1}{c|}{\textbf{16.517}} &
%   \textbf{0.909} &
%   \multicolumn{1}{c|}{85.50} &
%   \multicolumn{1}{c|}{64.21} &
%   \multicolumn{1}{c|}{-} &
%   - \\ \hline
% \end{tabular}
% }
% \caption{Overall Evaluation Results on e-SNLI and ComVE datasets of T5-based and BART-based \sage (Our \method method with \sage as the graph layer). The best performance of each evaluation metric across all NLE generation models of \textcolor{red}{the same base model architecture} is in bold.}
% \label{tab:all_results_all_datasets_bart}
% \end{table*}






% \begin{table*}[ht]
% \centering
% \small
% \normalsize
% \scalebox{0.48}{
% \begin{tabular}{@{}lcc|cccc|cccc@{}}
% \toprule
% \multicolumn{1}{c}{} &
%   \multicolumn{2}{c|}{Datasets} &
%   \multicolumn{4}{c|}{e-SNLI} &
%   \multicolumn{4}{c}{ComVE} \\ \midrule
%  &
%   \multicolumn{2}{c|}{\multirow{2}{*}{Evaluation Metrics}} &
%   \multicolumn{2}{c|}{Unfaithfulness (\% $\downarrow$)} &
%   \multicolumn{2}{c|}{Automatic Evaluation ($\uparrow$)} &
%   \multicolumn{2}{c|}{Unfaithfulness (\% $\downarrow$)} &
%   \multicolumn{2}{c}{Automatic Evaluation ($\uparrow$)} \\ \cmidrule(lr){4-11} 
%  &
%   \multicolumn{2}{c|}{} &
%   \multicolumn{1}{c|}{Counter Unfaith} &
%   \multicolumn{1}{c|}{Total Unfaith} &
%   \multicolumn{1}{c|}{SacreBLEU (0-100)} &
%   BERTScore (0-1) &
%   \multicolumn{1}{c|}{Counter Unfaith} &
%   \multicolumn{1}{c|}{Total Unfaith} &
%   \multicolumn{1}{c|}{SacreBLEU (0-100)} &
%   BERTScore (0-1) \\ \midrule
% \multirow{7}{*}{T5} &
%   \multicolumn{2}{c|}{Fine-tuning} &
%   47.08 & 16.89 & 15.430 & 0.894 &
%   \textbf{87.17} & 73.73 & - & - \\ \cmidrule(lr){2-11}
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{Highlight Token Explanation}} &
%   Prompt &
%   42.04 & 14.11 & 15.686 & 0.898 &
%   87.04 & 74.18 & - & - \\ \cmidrule(lr){3-11}
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   33.45 & 10.47 & 16.426 & \textbf{0.908} &
%   90.44 & \textbf{56.59} & - & - \\ \cmidrule(lr){2-11}
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{Token Interactive Explanation}} &
%   Prompt &
%   51.56 & 19.20 & 15.478 & 0.898 &
%   87.36 & 76.43 & - & - \\ \cmidrule(lr){3-11}
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   33.68 & 10.40 & \textbf{16.443} & \textbf{0.908} &
%   91.11 & 76.41 & - & - \\ \cmidrule(lr){2-11}
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{Span Interactive Explanation}} &
%   Prompt &
%   42.47 & 13.65 & 16.031 & 0.899 &
%   89.34 & 79.44 & - & - \\ \cmidrule(lr){3-11}
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \textbf{32.07} & \textbf{10.02} & 16.277 & 0.907 &
%   92.15 & 70.97 & - & - \\ \midrule
% \multirow{7}{*}{BART} &
%   \multicolumn{2}{c|}{Fine-tuning} &
%   57.98 & 19.64 & 15.732 & 0.906 &
%   \textbf{82.72} & 72.82 & - & - \\ \cmidrule(lr){2-11}
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{Highlight Token Explanation}} &
%   Prompt &
%   56.65 & 24.20 & 15.678 & 0.898 &
%   84.74 & 61.97 & - & - \\ \cmidrule(lr){3-11}
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   46.36 & \textbf{14.37} & 16.318 & \textbf{0.909} &
%   92.99 & \textbf{57.81} & - & - \\ \cmidrule(lr){2-11}
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{Token Interactive Explanation}} &
%   Prompt &
%   51.56 & 19.20 & 15.478 & 0.898 &
%   95.85 & 69.86 & - & - \\ \cmidrule(lr){3-11}
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   47.55 & 15.55 & 16.427 & \textbf{0.909} &
%   97.18 & 72.52 & - & - \\ \cmidrule(lr){2-11}
%  &
%   \multicolumn{1}{c|}{\multirow{2}{*}{Span Interactive Explanation}} &
%   Prompt &
%   51.10 & 17.41 & 16.027 & \textbf{0.909} &
%   94.89 & 65.52 & - & - \\ \cmidrule(lr){3-11}
%  &
%   \multicolumn{1}{c|}{} &
%   \sage (Ours) &
%   \textbf{44.42} & 14.56 & \textbf{16.517} & \textbf{0.909} &
%   85.50 & 64.21 & - & - \\ \bottomrule
% \end{tabular}
% }
% \caption{Overall evaluation results on e-SNLI and ComVE datasets for T5-based and BART-based models. \sage refers to our method using \sage as the graph layer. The best performance of each evaluation metric across all NLE generation models of the same base architecture is in bold.}
% \label{tab:all_results_all_datasets_bart}
% \end{table*}

